UniWeTok: An Unified Binary Tokenizer with Codebook Size $\mathit{2^{128}}$ for Unified Multimodal Large Language Model

Unified Multimodal Large Language Models (MLLMs) require a visual representation that simultaneously supports high-fidelity reconstruction, complex semantic extraction, and generative suitability. However, existing visual tokenizers typically struggle to satisfy these conflicting objectives within a single framework. In this paper, we introduce UniWeTok, a unified discrete tokenizer designed to bridge this gap using a massive binary codebook ($\mathit{2^{128}}$). For training framework, we introduce Pre-Post Distillation and a Generative-Aware Prior to enhance the semantic extraction and generative prior of the discrete tokens. In terms of model architecture, we propose a convolution-attention hybrid architecture with the SigLu activation function. SigLu activation not only bounds the encoder output and stabilizes the semantic distillation process but also effectively addresses the optimization conflict between token entropy loss and commitment loss. We further propose a three-stage training framework designed to enhance UniWeTok's adaptability cross various image resolutions and perception-sensitive scenarios, such as those involving human faces and textual content. On ImageNet, UniWeTok achieves state-of-the-art image generation performance (FID: UniWeTok 1.38 vs. REPA 1.42) while requiring a remarkably low training compute (Training Tokens: UniWeTok 33B vs. REPA 262B). On general-domain, UniWeTok demonstrates highly competitive capabilities across a broad range of tasks, including multimodal understanding, image generation (DPG Score: UniWeTok 86.63 vs. FLUX.1 [Dev] 83.84), and editing (GEdit Overall Score: UniWeTok 5.09 vs. OmniGen 5.06). We release code and models to facilitate community exploration of unified tokenizer and MLLM.

==> sections/preliminary.tex <==
\section{Preliminary}

\label{sec:preliminary}
% @liang init
% @tianshun supplement
% Many language-based reasoning tasks can be framed as sequential decision-making problems, where a policy must learn to generate correct answers through sparse feedback. These settings are typically modeled as Markov Decision Processes (MDPs), defined by the tuple $(\mathcal{S}, \mathcal{A}, P, r, \gamma)$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ the action space, $P$ the transition dynamics, $r$ the reward function, and $\gamma \in (0,1)$ the discount factor. The goal is to learn a policy $\pi$ that maximizes the expected return:
% $$
% \mathbb{E}_\pi \left[\sum_t \gamma^t r(s_t,a_t)\right].
% $$

% In our setting, the environment corresponds to the autoregressive generation behavior of a language model. More formally, we define:

% \begin{description}
%     \item[States ($\mathcal{S}$)] A state $s_t = (x_0, \dots, x_m, y_0, \dots, y_t)$ represents the full input–output sequence prefix up to time step $t$, where $x_{0:m}$ denotes the input context (e.g., question) and $y_{0:t}$ the generated output tokens so far.
    
%     \item[Actions ($\mathcal{A}$)] An action $a = y_{t+1} \in \mathcal{V}$ corresponds to selecting the next token from a fixed vocabulary $\mathcal{V}$.
    
%     \item[Dynamics ($\mathbb{P}$)] These represent a deterministic transition model between tokens. Given a state $s_t = (x_0, \dots, x_m, y_0, \dots, y_t)$, an action $a = y_{t+1}$, and the subsequent state $s_{t+1} = (x_0, \dots, x_m, y_0, \dots, y_t, y_{t+1})$, the probability $\mathbb{P}(s_{t+1} \mid s_t, a) = 1$.
    
%     \item[Reward ($r$)] Rewards are typically sparse in generation task. This sparsity stems from the fact that meaningful evaluation can only be performed at the end of a complete rollout, after the final token has been generated. Consequently, the llm receives no intermediate feedback during the generation process, which severely limits the availability of informative signals for policy updates and poses a major challenge for exploration.
% \end{description}
\subsection{MDP Setup for Autoregressive Generation}
Many language-based reasoning tasks can be naturally formulated as sequential decision-making problems, modeled as Markov Decision Processes (MDPs). An MDP is defined by the tuple \((\mathcal{S}, \mathcal{A}, P, r, \gamma)\), where \(\mathcal{S}\) is the state space, \(\mathcal{A}\) the action space, \(P\) the transition dynamics, \(r\) the reward function, and \(\gamma \in (0,1)\) the discount factor~\citep{sutton1998reinforcement}. The objective is to learn a policy \(\pi\) that maximizes the expected return:
\begin{equation}
\mathbb{E}_\pi \left[\sum_t \gamma^t r(s_t, a_t)\right]
\end{equation}

In the context of large language models (LLMs), the environment corresponds to the autoregressive generation process~\citep{81a0972a0b704d918ec2ce3696c5b871,ouyang2022training}. Specifically:

\textbf{States (\(\mathcal{S}\)):} Each state \(s_t = (x_0, \dots, x_m, y_0, \dots, y_t)\) includes the input context \(x_{0:m}\) and the generated tokens \(y_{0:t}\).

\textbf{Actions (\(\mathcal{A}\)):} An action \(a = y_{t+1} \in \mathcal{V}\) corresponds to selecting the next token from the vocabulary \(\mathcal{V}\).

\textbf{Dynamics (\(P\)):} The environment transitions deterministically to \(s_{t+1} = (x_0, \dots, x_m, y_0, \dots, y_{t+1})\).

\textbf{Reward (\(r\)):} Rewards are typically sparse, provided only at the end of a complete rollout, limiting intermediate feedback and posing challenges for effective exploration~\citep{schulman2017proximalpolicyoptimizationalgorithms}.



\subsection{Rejection Sampling}

In the stage of advantage estimating, when a prompt consistently yields trajectories with identical rewards, either all correct (reward = 1) or all incorrect (reward = 0), the corresponding advantage estimates become zero. This leads to vanishing policy gradients and results in reduced sample efficiency. As training progresses, more prompts fall into this degenerate category, causing the effective batch size to shrink and increasing the variance of gradient estimates.

To mitigate this issue during our \textit{entropy finding} phase—which aims to identify uncertain reasoning positions for structured exploration—we employ \textit{rejection sampling}~\citep{yu2025dapoopensourcellmreinforcement,zhang2025srpocrossdomainimplementationlargescale}. Specifically, for each prompt, we perform multiple rollouts and compute their corresponding binary rewards. If all rollouts yield the same reward (i.e., either all 0s or all 1s), the prompt is considered degenerate and is rejected from the current batch. This ensures that the entropy-finding process operates on diverse and informative reasoning trajectories, rather than being misled by degenerate cases with no variation in reward.


\subsection{Clip-Higher}
Standard PPO-based reinforcement learning constrains policy updates using symmetric clipping bounds, typically limiting the probability ratio $r_{i,t}(\theta)$ within $[0.8, 1.2]$ to prevent unstable updates. However, this symmetric structure also suppresses the probability growth of low-confidence tokens, which hinders exploration and can lead to \textit{entropy collapse}---a state where the policy becomes overly deterministic and loses action diversity.

To address this issue and explicitly encourage exploration, we adopt the \textit{Clip-Higher} mechanism~\citep{yue2025vapoefficientreliablereinforcement}, which replaces symmetric clipping with asymmetric bounds that permit more substantial increases in the probability of underexplored but potentially valuable reasoning paths, while still limiting overly aggressive decreases. This asymmetry encourages the policy to better explore less probable trajectories without sacrificing training stability. Empirical validation in our setting shows that this design improves both exploration efficiency and learning robustness. We use $\epsilon_{\text{low}} = 0.22$ and $\epsilon_{\text{high}} = 0.28$, yielding the objective:
\begin{equation}
\mathcal{L}_{\text{PPO}}(\theta) =
-\frac{1}{\sum_{i=1}^G |o_i|}
\sum_{i=1}^G \sum_{t=1}^{|o_i|}
\min\left(
r_{i,t}(\theta) \hat{A}_{i,t},~
\text{clip}(r_{i,t}(\theta), 1 - \epsilon_{\text{low}}, 1 + \epsilon_{\text{high}}) \hat{A}_{i,t}
\right)
\end{equation}
This asymmetrically clipped objective plays a key role in preserving policy diversity and enhancing long-horizon reasoning through more effective exploration.



% \subsection{Structured Exploration}

% The principle of structured exploration, which involves systematically revisiting and expanding upon promising partial solutions, has demonstrated considerable efficacy in reinforcement learning, exemplified by seminal approaches like Go-Explore~\citep{Ecoffet_2021}. This paradigm is particularly pertinent to LLMs operating in complex reasoning tasks characterized by sparse and delayed rewards. In such scenarios, conventional random exploration often proves inefficient, failing to identify or adequately exploit critical intermediate reasoning steps that are essential for reaching optimal solutions.

% To address this limitation, we investigate a targeted, two-stage exploration strategy. The initial stage focuses on identifying high-uncertainty decision points within nascent reasoning trajectories. These points, often corresponding to local minima in token-level log-probabilities, signify potential junctures or critical forks in the reasoning process and are designated as intermediate reasoning states. In the subsequent stage, these identified intermediate states are systematically revisited, and controlled partial rollouts are initiated from them to expand upon the existing reasoning paths. This structure provide a principled framework for navigating the reasoning space of LLMs, enabling the model to build upon promising partial solutions while efficiently discovering new, high-reward trajectories.

\subsection{Structured Exploration}
Our methodology is inspired by the principles of structured exploration, particularly the ``First Return, Then Explor'' paradigm popularized by Go-Explore~\citep{Ecoffet_2021}. This approach has demonstrated considerable efficacy in tasks with sparse rewards by first focusing on finding a path to a novel state (the ``first return'') and only then initiating deeper exploration from that promising location. For complex reasoning tasks in LLMs, where random exploration is inefficient, this paradigm offers a more principled way to navigate the vast generation space.

We adapt this ``First Return, Then Explore'' principle for the autoregressive generation process of LLMs. The \textbf{``First Return''} phase involves generating initial, promising trajectories. Instead of exploring randomly, our \textbf{``Entropy-Eliciting Explore''} phase then analyzes these trajectories to pinpoint states of high model uncertainty. These states, often identified by local minima in token-level log-probabilities (i.e., high local entropy), represent critical junctures where the model is least confident. By systematically initiating partial rollouts from these high-entropy states, we can efficiently discover valuable alternative reasoning paths and generate dense, informative feedback, enabling the model to build upon promising solutions in a targeted manner.

==> tables/ablation_ar_prior.tex <==
\begin{table}[t]
    \centering
    \tablestyle{5pt}{1.1}
    \caption{\textbf{Effectiveness of AR Prior Loss on ImageNet.} The generative prior improves gFID while maintaining high reconstruction quality.}
    \label{tab:ar_prior}
    \begin{tabular}{l|c|cccc|cc}
        \toprule
        \rowcolor{graybg}
         & \textbf{Gen.} & \multicolumn{4}{c|}{\textbf{Reconstruction}} & \multicolumn{2}{c}{\textbf{Zero-shot Acc (\%)}} \\
        \rowcolor{graybg}
        \multirow{-2}{*}{Method} & gFID $\downarrow$ & rFID $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & \scriptsize{LPIPS(A)} & Top-1 & Top-5 \\
        \midrule
        w/o Prior Loss & 2.66 & \textcolor{bestblue}{\textbf{1.12}} & \textcolor{bestblue}{\textbf{22.32}} & \textcolor{bestblue}{\textbf{0.647}} & \textcolor{bestblue}{\textbf{0.122}} & 46.89 & 73.66 \\
        w/ Prior (no class) & 3.89 & 1.16 & 22.11 & 0.634 & 0.126 & 48.47 & 74.80 \\
        \textbf{w/ Prior (Class)} & \textcolor{bestblue}{\textbf{2.30}} & 1.18 & 22.27 & 0.632 & 0.124 & \textcolor{bestblue}{\textbf{48.77}} & \textcolor{bestblue}{\textbf{75.62}} \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/ablation_channel.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Effect of Downsample Channel Capacity.} Increasing the channel width in the bottleneck significantly enhances both reconstruction fidelity and semantic alignment.}
    \label{tab:channel}
    \resizebox{0.95\linewidth}{!}{
        \begin{tabular}{l|ccccc|ccc}
        \toprule
        \rowcolor{tabheader}
        & \multicolumn{5}{c|}{\textbf{Reconstruction Metrics}} & \multicolumn{3}{c}{\textbf{Zero-shot Acc (\%)}} \\
        \rowcolor{tabheader}
        \multirow{-2}{*}{\textsc{Method}} & rFID $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & \scriptsize{LPIPS(Alex)} & \scriptsize{LPIPS(VGG)} & Top-1 & Top-5 & Top-10 \\
        \midrule
        Single Channel & 1.58 & 21.89 & 0.626 & 0.131 & 0.225 & 39.45 & 68.00 & 76.77 \\
        \rowcolor{tabhighlight}
        \textbf{Double Channel} & \best{1.12} & \best{22.32} & \best{0.647} & \best{0.122} & \best{0.210} & \best{46.89} & \best{73.66} & \best{81.11} \\
        \bottomrule
        \end{tabular}
    }
\end{table}

==> tables/tab_combo_distill_channel.tex <==
\begin{table}[t]
    \centering
    % --- Left: Table 1 (Distillation Strategy) ---
    \begin{minipage}[b]{0.33\linewidth}
        \centering
        \tablestyle{2pt}{1.2}
        \caption{\textbf{Distillation strategy.} Effect of distillation loss and SigLu activation.}
        \label{tab:distill_strat}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{l|ccc}
                \toprule
                Method & Top-1 & Top-5 & Top-10 \\
                \midrule
                \rowcolor{rowgray}
                Pre Distill & 55.26 & 79.55 & 85.52 \\
                Post Distill & 0.10 & 0.53 & 0.95 \\
                \rowcolor{bestblue} \textbf{SigLu + Post} & \textbf{41.51} & \textbf{69.51} & \textbf{77.73} \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
    \hfill
    % --- Right: Table 3 (Channel Capacity) ---
    \begin{minipage}[b]{0.65\linewidth}
        \centering
        \tablestyle{1pt}{1.2}
        \caption{\textbf{Bottleneck channel.} Increasing channel width of bottleneck significantly improves fidelity and alignment.}
        \label{tab:channel}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{l|ccccc|ccc}
                \toprule
                & \multicolumn{5}{c|}{\textbf{Reconstruction Metrics}} & \multicolumn{3}{c}{\textbf{Zero-shot Acc (\%)}} \\
                \multirow{-2}{*}{Method} & rFID$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & \tiny{LPIPS(A)}$\downarrow$ & \tiny{LPIPS(V)}$\downarrow$ & Top-1 & Top-5 & Top-10 \\
                \midrule
                Single Chan. & 1.58 & 21.89 & 0.626 & 0.131 & 0.225 & 39.45 & 68.00 & 76.77 \\
                \rowcolor{bestblue} \textbf{Double Chan.} & \textbf{1.12} & \textbf{22.32} & \textbf{0.647} & \textbf{0.122} & \textbf{0.210} & \textbf{46.89} & \textbf{73.66} & \textbf{81.11} \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{table}

==> tables/tab_combo_loss_prior.tex <==
\begin{table}[!ht]
    \centering
    % --- Left: Table 2 (Loss Necessity with Checkmarks) ---
    \begin{minipage}[b]{0.355\linewidth}
        \centering
        \tablestyle{4pt}{1.2}
        \caption{\textbf{Loss Necessity.} Dual-stage loss yields the best performance.}
        \label{tab:distill_loss}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{cc|ccc}
                \toprule
                \multicolumn{2}{c|}{\textbf{Distillation Loss}} & \multicolumn{3}{c}{\textbf{Zero-shot Acc (\%)}} \\
                \textsc{Pre} & \textsc{Post} & Top-1 & Top-5 & Top-10 \\
                \midrule
                \cmark & \xmark & 0.10 & 0.52 & 1.01 \\
                \xmark & \cmark & 41.51 & 69.51 & 77.73 \\
                \rowcolor{bestblue} \cmark & \cmark & \textbf{51.32} & \textbf{76.70} & \textbf{83.26} \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
    \hfill
    % --- Right: Table 4 (AR Prior) ---
    \begin{minipage}[b]{0.625\linewidth}
        \centering
        \tablestyle{1pt}{1.2}
        \caption{\textbf{AR Prior Loss.} Generative prior loss significantly improves gFID while maintaining reconstruction and semantic extraction.}
        \label{tab:ar_prior}
        \resizebox{\linewidth}{!}{
            \begin{tabular}{cc|c|ccccc|ccc}
                \toprule
                \multicolumn{2}{c|}{\textbf{Method}}
                & \textbf{Gen.} & \multicolumn{5}{c|}{\textbf{Reconstruction}} & \multicolumn{3}{c}{\textbf{Zero-shot Acc (\%)}} \\
                \textsc{Prior} & \textsc{Cls} & gFID$\downarrow$ & rFID$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & \tiny{LPIPS(A)}$\downarrow$ & \tiny{LPIPS(V)}$\downarrow$ & Top-1 & Top-5 & Top-10 \\
                \midrule
                \xmark & \xmark & 2.66 & \textbf{1.12} & \textbf{22.32} & \textbf{0.647} & \textbf{0.122} & \textbf{0.210} & 46.89 & 73.66 & 81.11 \\
                \cmark & \xmark & 3.89 & 1.16 & 22.11 & 0.634 & 0.126 & 0.218 & 48.47 & 74.80 & 82.23 \\
                \rowcolor{bestblue} \cmark & \cmark & \textbf{2.38} & 1.18 & 22.27 & 0.632 & 0.124 & 0.218 & \textbf{48.77} & \textbf{75.62} & \textbf{83.84} \\
                \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{table}
